A Scalable Approach for Privacy-Preserving Collaborative Machine Learning

We consider a collaborative learning scenario in which multiple data-owners wish to jointly train a logistic regression model, while keeping their individual datasets private from the other parties. We propose COPML, a fully-decentralized training framework that achieves scalability and privacy-protection simultaneously. The key idea of COPML is to securely encode the individual datasets to distribute the computation load effectively across many parties and to perform the training computations as well as the model updates in a distributed manner on the securely encoded data. We provide the privacy analysis of COPML and prove its convergence. Furthermore, we experimentally demonstrate that COPML can achieve significant speedup in training over the benchmark protocols. Our protocol provides strong statistical privacy guarantees against colluding parties (adversaries) with unbounded computational power, while achieving up to $16\times$ speedup in the training time against the benchmark protocols.

==> App_convergenceproof.tex <==
\hspace{-0.11cm}First, we show that the minimum number of clients needed for our decoding operation to be successful, i.e., the recovery threshold of {\acr}, is equal to $(2r+1)(K+T-1)+1$. 
To do so, we demonstrate in the following that the decoding process will be successful as long as $N\geq (2r+1)(K+T-1) +1$.  
% gradient $\bX^\top \hat{g}(\bX \times \bw^{(t)})$ from~\eqref{eq:agg} can be decoded as long as $N\geq (2r+1)(K+T-1) +1$. 
As described in Section~\ref{app:multiclient_framework}, given the polynomial approximation of the sigmoid function  in~\eqref{eq:poly_approximation}, the degree of $h(z)$ in~\eqref{eq:beta} is at most $(2r+1)(K+T-1)$. 
The decoding process uses the computations from the clients as evaluation points $h(\alpha_i)$ to interpolate the polynomial $h(z)$. 
% All of the coefficients of $h(z)$ can be evaluated by collecting at least $deg(h(z))+1$ evaluation results of $h(\alpha_i)$. 
If at least $deg(h(z))+1$ evaluation results of $h(\alpha_i)$ are available, then, all of the coefficients of $h(z)$ can be evaluated. 
After $h(z)$ is recovered, the sub-gradient $\bX_i^\top \hat{g}(\bX_i \times \bw^{(t)})$ can be decoded by computing $h(\beta_i)$ for $i\in[K]$, from which the gradient $\bX^\top \hat{g}(\bX \times \bw^{(t)})$ from \eqref{eq:agg} can be computed. 
Hence, the recovery threshold of {\acr} is  $(2r+1)(K+T-1) +1$, as long as $N\geq (2r+1)(K+T-1) +1$, the protocol can correctly decode the gradient using the local evaluations of the clients, and the decoding process will be successful. 
% As described in Section~\ref{app:multiclient_framework},  the decoding operations are performed using a secure MPC protocol between the clients, as a result, throughout the decoding process, the clients only learn a secret share of the gradient and not its actual value. 
% As described in Section~\ref{app:multiclient_framework},  
Since the decoding operations are performed using a secure MPC protocol, throughout the decoding process, the clients only learn a secret share of the gradient and not its actual value. 
% {\color{red}
% This is enabled by the fact that our decoding process corresponds to a  finite-field polynomial interpolation problem, which can be solved through finite-field polynomial evaluations by using a secure MPC protocol.}
% 
% 
% We note that this decoding process and updating the model as in~\eqref{eq:apprx_grad1multi} take place in a secure MPC protocol, i.e., each client only learns a secret share of the final computation $\bX^\top \big(\hat{g}(\bX \times \bw^{(t)})-\mathbf{y}\big)$ and a secret share of updated model $\bw^{(t+1)}$. 
Next, we consider the update equation in \eqref{eq:apprx_grad1multi} and prove its convergence to $\mathbf{w}^*$.
As described in Section~\ref{app:multiclient_framework}, after decoding the gradient, the clients carry out a secure truncation protocol to multiply $\bX^\top (\hat{g}(\bX \times \bw^{(t)})-\mathbf{y})$ with parameter $\frac{\eta}{m}$ to update the model as in~\eqref{eq:apprx_grad1multi}.
% The truncation protocol introduces a quantization noise to the update process, which we represent by $\mathbf{v}^{(t)}$. 
The update equation from \eqref{eq:apprx_grad1multi} can then be represented by
\begin{align}
    \bw^{(t+1)}  &=   \bw^{(t)}\!-\eta \big(\frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{n}^{(t)} \big). \label{eq:updateEQN_secret}\\
    &=\bw^{(t)}\!-\eta \mathbf{p}^{(t)} \label{eq:define_p}
\end{align}
where $\mathbf{n}^{(t)}$ represents the quantization noise introduced by the secure multi-party truncation protocol ~\cite{catrina2010secure}, and $\mathbf{p}^{(t)} \triangleq \frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{n}^{(t)}$. 
% denotes the gradient computation of {\acr}.
From~\cite{catrina2010secure}, $\mathbf{n}^{(t)}$ has zero mean and bounded variance, i.e., $\mathbb{E}[\mathbf{n}^{(t)}]=0$ and $\mathbb{E}\big[\| \mathbf{n}^{(t)}  \|^{2}_{2} \big] \leq \frac{d2^{2(k_1-1)}}{m^2} \triangleq \sigma^2$ where $\| \cdot \|_{2}$ is the $l_2$ norm and $k_1$ is the truncation parameter described in Section~\ref{app:multiclient_framework}.
% Then, we can prove that $\mathbf{p}^{(t)}$ is unbiased and variance bounded with sufficiently large $r$. 

Next, we show that $\mathbf{p}^{(t)}$ is an unbiased estimator of the true gradient, $\nabla C(\bw^{(t)})=\frac{1}{m} {\mathbf{X}}^{\top} (g({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})$, and its variance is bounded by $\sigma^2$ with sufficiently large $r$.
% From $\mathbb{E}[\mathbf{v}^{(t)}]=0$,
% Unbiasedness of $\mathbf{p}^{(t)}$ follows from $\mathbb{E}[\mathbf{v}^{(t)}]=0$, i.e., $\mathbb{E}[\mathbf{p}^{(t)}]  = \frac{1}{m} {\bX}^{\top} \big( \hat{g}({\bX} \times {\bw}^{(t)}) - \mathbf{y} \big)=\nabla C(\bw^{(t)})$.
% \begin{equation}
% \mathbb{E}[\mathbf{p}^{(t)}]  = \frac{1}{m} {\bX}^{\top} \Big( \hat{g}({\bX} \times {\bw}^{(t)}) - \mathbf{y} \Big) \label{eq:unb}
% \end{equation}
% due to the unbiasedness of the truncation protocol. 
From $\mathbb{E}[\mathbf{n}^{(t)}]=0$, we obtain
\begin{equation}\label{eq:delta}
    \mathbb{E}[\mathbf{p}^{(t)}] - \nabla C(\bw^{(t)}) =\frac{1}{m}\bX^{\top} \big( \hat{g}({\bX}\times {\bw}^{(t)}) - g({\bX}\times {\bw}^{(t)}) \big).  
\end{equation}
From the Weierstrass approximation theorem~\cite{brinkhuis2011optimization}, for any $\epsilon>0$, there exists a polynomial that approximates the sigmoid arbitrarily well, i.e., $|\hat{g}(x)-g(x)|\leq\epsilon$ for all $x$ in the constrained interval.  
% The domain for the sigmoid function is bounded as $\|\bw\|\leq R$. 
Hence, as there exists a polynomial making the norm of~\eqref{eq:delta} arbitrarily small, $\mathbb{E}[\mathbf{p}^{(t)}]=\nabla C(\bw^{(t)})$ and $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{n}^{(t)}  \|^{2}_{2} \big] \leq \sigma^2$. 
% The variance of $\mathbf{p}^{(t)}$ is bounded as $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)}  \|^{2}_{2} \big] \leq \sigma^2$.
% In addition, the variance of $\mathbf{p}^{(t)}$ is bounded as $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)} - \mathbb{E}[\mathbf{v}^{(t)}] \|^{2}_{2} \big] \leq \sigma^2$.

% Let $\mathbf{p}^{(t)} \triangleq \frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}}, {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{v}^{(t)}$ denote the gradient computation of {\acr}. 
% Then, one can show that, (unbiasedness) $\mathbb{E}[\mathbf{p}^{(t)}] = \nabla C (\bw^{(t)})+ \epsilon(r) $ where $\epsilon(r)\rightarrow \mathbf{0}$ as $r\rightarrow\infty$ (see Weierstrass approximation theorem~\cite{brinkhuis2011optimization}) and the expectation is taken with respect to the quantization noises, and (variance bound) $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)} - \mathbb{E}[\mathbf{v}^{(t)}] \|^{2}_{2} \big] \leq \sigma^2$.



% (Convergence)
% Next, we consider the update equation in {\acr} from~\eqref{eq:updateEQN_secret} and prove its convergence to $\bw^{*}$. From the $L$-Lipschitz continuity of $\nabla C({\bw})$ stated in where $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$, we have
Next, we consider the update equation in~\eqref{eq:define_p} and prove its convergence to $\bw^{*}$. From the $L$-Lipschitz continuity of $\nabla C({\bw})$ 
(Theorem 2.1.5 of~\cite{book_Nesterov}), we have
% the gradient of the cross entropy loss function, $\nabla C({\bw})$, we have
\begin{align}
    C(\bw^{(t+1)}) 
    &\!\leq \!C(\bw^{(t)}) \!+\! \langle \nabla C(\bw^{(t)}), \bw^{(t+1)}\!-\!\bw^{(t)}\rangle 
    \!+\! \frac{L}{2}{\| \bw^{(t+1)}\!-\!\bw^{(t)}\! \|}^2  \notag\\
    &\!\leq\! C( \bw^{(t)} )\!-\!\eta \langle \gC ( \bw^{(t)} ), \mathbf{p}^{(t)} \rangle + \frac{L\eta^2}{2}{\| \mathbf{p}^{(t)} \|}^2, \label{eq:Lipschitz_ineq}
\end{align} 
% where $\langle ,\cdot, \rangle$ is the inner product and $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$.
where $\langle ,\cdot, \rangle$ is the inner product. For a cross entropy loss $C(\bw)$, the Lipschitz
constant $L$ is equal to the largest eigenvalue of the Hessian $\nabla^2C(\bw)$ for all $\bw$, and is given by $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$.
By taking the expectation with respect to the quantization noise on both sides in~\eqref{eq:Lipschitz_ineq}, we have
\begin{align}
    \mathbb{E}\big[ C(\bw^{(t+1)}) \big] 
    &\leq C( \bw^{(t)} ) - \eta \| \gC ( \bw^{(t)} )\|^2 +\frac{L\eta^2}{2} \big( \| \gC ( \bw^{(t)} )\|^2 + \sigma^2 \big) \label{eq:fisrt_ineq} \\
    &\leq C( \bw^{(t)} ) - \eta \big(1-\frac{L\eta}{2}\big)\| \gC ( \bw^{(t)} )\|^2+\frac{L\eta^2\sigma^2}{2} \notag \\
    &\leq C( \bw^{(t)} ) - \frac{\eta}{2}\| \gC ( \bw^{(t)} )\|^2\!+\!\frac{\eta\sigma^2}{2} \label{eqn1} \\
    &\leq C(\bw^{*})\!+\!\langle \gC ( \bw^{(t)} ), \bw^{(t)} \!-\! \bw^{*}\rangle 
    - \frac{\eta}{2} \| \gC ( \bw^{(t)} )\|^2\!+\!\frac{\eta\sigma^2}{2} \label{eqn2}\\
    &\leq C(\bw^{*})+ \langle\mathbb{E}[\mathbf{p}^{(t)}],\bw^{(t)} - \bw^{*}\rangle - \frac{\eta}{2} \mathbb{E}\big[\| \mathbf{p}^{(t)} )\|^2\big]+\eta\sigma^2 \label{eqn3}\\
    &= C(\bw^{*}) +\eta\sigma^2 +\mathbb{E}\Big[ \langle \mathbf{p}^{(t)},\bw^{(t)}-\bw^{*} \rangle-\frac{\eta}{2}\| \mathbf{p}^{(t)} )\|^2\Big] \notag \\
    &=\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \| \bw^{(t)} - \bw^{*} \|^2 -\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
    % &\leq\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \| \bw^{(t)} - \bw^{*} \|^2 -\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
\end{align}
where~\eqref{eq:fisrt_ineq} and~\eqref{eqn3} hold since  $\mathbb{E}[\mathbf{p}^{(t)}]=\nabla C(\bw^{(t)})$ and $\mathbb{E}\big[\| \mathbf{p}^{(t)}  - \nabla C(\bw^{(t)}) \|^{2}_{2} \big] \leq \sigma^2$,~\eqref{eqn1} follows from $L\eta\leq1$, and~\eqref{eqn2} follows from the convexity of $C$.
% where~\eqref{eq:fisrt_ineq} and~\eqref{eqn3} hold since  $\mathbb{E}[\mathbf{p}^{(t)}]=\nabla C(\bw^{(t)})$ and $\mathbb{E}\big[\| \mathbf{p}^{(t)}  - \nabla C(\bw^{(t)}) \|^{2}_{2} \big] \leq \sigma^2$,~\eqref{eqn1} follows from $L\eta\leq1$,~\eqref{eqn2} follows from the convexity of $C$, and \eqref{eqn4} holds since $2\langle \mathbf{a},\mathbf{b}\rangle \leq \| \mathbf{a} \|^2_2 + \| \mathbf{b} \|^2_2$ for any vector $\mathbf{a}$ and $\mathbf{b}$.

% {\color{blue}
% By taking the expectation on both sides in~\eqref{eq:Lipschitz_ineq} with respect to the quantization noises $\mathbf{n}^{(t)}$ for $t=0,\ldots,J-1$ where $J$ denotes the total number of iterations, we have
% \begin{align}
%     \mathbb{E}\big[ C(\bw^{(t+1)}) \big] 
%     &\leq \mathbb{E}\big[C( \bw^{(t)} )\big] - \eta \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big] +\frac{L\eta^2}{2} \big( \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big] + \sigma^2 \big) \label{eq:fisrt_ineq} \\
%     &\leq C( \bw^{(t)} ) - \eta \big(1-\frac{L\eta}{2}\big)\| \gC ( \bw^{(t)} )\|^2+\frac{L\eta^2\sigma^2}{2} \notag \\
%     &\leq C( \bw^{(t)} ) - \frac{\eta}{2}\| \gC ( \bw^{(t)} )\|^2\!+\!\frac{\eta\sigma^2}{2} \label{eqn1} \\
%     &\leq C(\bw^{*})\!+\!\langle \gC ( \bw^{(t)} ), \bw^{(t)} \!-\! \bw^{*}\rangle 
%     - \frac{\eta}{2} \| \gC ( \bw^{(t)} )\|^2\!+\!\frac{\eta\sigma^2}{2} \label{eqn2}\\
%     &\leq C(\bw^{*})+ \langle\mathbb{E}[\mathbf{p}^{(t)}],\bw^{(t)} - \bw^{*}\rangle - \frac{\eta}{2} \mathbb{E}\big[\| \mathbf{p}^{(t)} )\|^2\big]+\eta\sigma^2 \label{eqn3}\\
%     &= C(\bw^{*}) +\eta\sigma^2 +\mathbb{E}\Big[ \langle \mathbf{p}^{(t)},\bw^{(t)}-\bw^{*} \rangle-\frac{\eta}{2}\| \mathbf{p}^{(t)} )\|^2\Big] \notag \\
%     &=\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \| \bw^{(t)} - \bw^{*} \|^2 -\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
%     % &\leq\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \| \bw^{(t)} - \bw^{*} \|^2 -\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
% \end{align}
% where~\eqref{eq:fisrt_ineq} and~\eqref{eqn3} hold since  $\mathbb{E}[\mathbf{p}^{(t)}]=\nabla C(\bw^{(t)})$ and $\mathbb{E}\big[\| \mathbf{p}^{(t)}  - \nabla C(\bw^{(t)}) \|^{2}_{2} \big] \leq \sigma^2$,~\eqref{eqn1} follows from $L\eta\leq1$,~\eqref{eqn2} follows from the convexity of $C$.
% }

Summing both sides of the inequality in~\eqref{eqn4} for $t=0,\ldots,J-1$, where $J$ denotes the total number of iterations, we find that,
\begin{align*}
    \sum_{t=0}^{J-1}\Big(\mathbb{E}\big[ &C(\bw^{(t+1)})\big]\!-\!C(\bw^{*})\Big) 
    % \notag \\
    % & \leq \frac{1}{2\eta}\big( \| \bw^{(0)} - \bw^{*} \|^2 -\| \bw^{(J)} - \bw^{*} )\|^2\big) + J\eta\sigma^2\\
    \leq \frac{\| \bw^{(0)} - \bw^{*} \|^2}{2\eta}\!+\!J\eta\sigma^2.
\end{align*}
Finally, since $C$ is convex, we observe that, 
\begin{align*}
    \mathbb{E}\Big[ C\big( \frac{1}{J}\sum_{t=0}^{J}\bw^{(t)}\big)\Big]\!-\!C(\bw^{*})
    &\leq \frac{1}{J} \sum_{t=0}^{J-1}\Big(\mathbb{E}\big[ C(\bw^{(t+1)})\big]\!-\!C(\bw^{*})\Big) \notag \\
    &\leq \frac{\| \bw^{(0)} - \bw^{*} \|^2}{2\eta J} + \eta\sigma^2%, 
\end{align*}
which completes the proof of convergence.

==> App_convergenceproof_v2.tex <==
\hspace{-0.11cm}First, we show that the minimum number of clients needed for our decoding operation to be successful, i.e., the recovery threshold of {\acr}, is equal to $(2r+1)(K+T-1)+1$. 
To do so, we demonstrate in the following that the decoding process will be successful as long as $N\geq (2r+1)(K+T-1) +1$.  
% gradient $\bX^\top \hat{g}(\bX \times \bw^{(t)})$ from~\eqref{eq:agg} can be decoded as long as $N\geq (2r+1)(K+T-1) +1$. 
As described in Section~\ref{app:multiclient_framework}, given the polynomial approximation of the sigmoid function  in~\eqref{eq:poly_approximation}, the degree of $h(z)$ in~\eqref{eq:beta} is at most $(2r+1)(K+T-1)$. 
The decoding process uses the computations from the clients as evaluation points $h(\alpha_i)$ to interpolate the polynomial $h(z)$. 
% All of the coefficients of $h(z)$ can be evaluated by collecting at least $deg(h(z))+1$ evaluation results of $h(\alpha_i)$. 
If at least $deg(h(z))+1$ evaluation results of $h(\alpha_i)$ are available, then, all of the coefficients of $h(z)$ can be evaluated. 
After $h(z)$ is recovered, the sub-gradient $\bX_i^\top \hat{g}(\bX_i \times \bw^{(t)})$ can be decoded by computing $h(\beta_i)$ for $i\in[K]$, from which the gradient $\bX^\top \hat{g}(\bX \times \bw^{(t)})$ from \eqref{eq:agg} can be computed. 
Hence, the recovery threshold of {\acr} is  $(2r+1)(K+T-1) +1$, as long as $N\geq (2r+1)(K+T-1) +1$, the protocol can correctly decode the gradient using the local evaluations of the clients, and the decoding process will be successful. 
% As described in Section~\ref{app:multiclient_framework},  the decoding operations are performed using a secure MPC protocol between the clients, as a result, throughout the decoding process, the clients only learn a secret share of the gradient and not its actual value. 
% As described in Section~\ref{app:multiclient_framework},  
Since the decoding operations are performed using a secure MPC protocol, throughout the decoding process, the clients only learn a secret share of the gradient and not its actual value. 
% {\color{red}
% This is enabled by the fact that our decoding process corresponds to a  finite-field polynomial interpolation problem, which can be solved through finite-field polynomial evaluations by using a secure MPC protocol.}
% 
% 
% We note that this decoding process and updating the model as in~\eqref{eq:apprx_grad1multi} take place in a secure MPC protocol, i.e., each client only learns a secret share of the final computation $\bX^\top \big(\hat{g}(\bX \times \bw^{(t)})-\mathbf{y}\big)$ and a secret share of updated model $\bw^{(t+1)}$. 
Next, we consider the update equation in \eqref{eq:apprx_grad1multi} and prove its convergence to $\mathbf{w}^*$.
As described in Section~\ref{app:multiclient_framework}, after decoding the gradient, the clients carry out a secure truncation protocol to multiply $\bX^\top (\hat{g}(\bX \times \bw^{(t)})-\mathbf{y})$ with parameter $\frac{\eta}{m}$ to update the model as in~\eqref{eq:apprx_grad1multi}.
% The truncation protocol introduces a quantization noise to the update process, which we represent by $\mathbf{v}^{(t)}$. 
The update equation from \eqref{eq:apprx_grad1multi} can then be represented by
\begin{align}
    \bw^{(t+1)}  &=   \bw^{(t)}\!-\eta \big(\frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{n}^{(t)} \big). \label{eq:updateEQN_secret}\\
    &=\bw^{(t)}\!-\eta \mathbf{p}^{(t)} \label{eq:define_p}
\end{align}
where $\mathbf{n}^{(t)}$ represents the quantization noise introduced by the secure multi-party truncation protocol ~\cite{catrina2010secure}, and $\mathbf{p}^{(t)} \triangleq \frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{n}^{(t)}$. 
% denotes the gradient computation of {\acr}.
From~\cite{catrina2010secure}, $\mathbf{n}^{(t)}$ has zero mean and bounded variance, i.e., $\mathbb{E}[\mathbf{n}^{(t)}]=0$ and $\mathbb{E}\big[\| \mathbf{n}^{(t)}  \|^{2}_{2} \big] \leq \frac{d2^{2(k_1-1)}}{m^2} \triangleq \sigma^2$ where $\| \cdot \|_{2}$ is the $l_2$ norm and $k_1$ is the truncation parameter described in Section~\ref{app:multiclient_framework}.
{\color{blue}Expectation is taken with respect to the quantization noises $\mathbf{n}^{(t)}$ for $t=0,\ldots,J-1$ where $J$ denotes the total number of iterations, and we assume that quantization noises are independent of each other.}
% Then, we can prove that $\mathbf{p}^{(t)}$ is unbiased and variance bounded with sufficiently large $r$. 

Next, we show that $\mathbf{p}^{(t)}$ is an unbiased estimator of the true gradient, $\nabla C(\bw^{(t)})=\frac{1}{m} {\mathbf{X}}^{\top} (g({\mathbf{X}} \times {\mathbf{w}}^{(t)}) -\mathbf{y})$, and its variance is bounded by $\sigma^2$ with sufficiently large $r$.
% From $\mathbb{E}[\mathbf{v}^{(t)}]=0$,
% Unbiasedness of $\mathbf{p}^{(t)}$ follows from $\mathbb{E}[\mathbf{v}^{(t)}]=0$, i.e., $\mathbb{E}[\mathbf{p}^{(t)}]  = \frac{1}{m} {\bX}^{\top} \big( \hat{g}({\bX} \times {\bw}^{(t)}) - \mathbf{y} \big)=\nabla C(\bw^{(t)})$.
% \begin{equation}
% \mathbb{E}[\mathbf{p}^{(t)}]  = \frac{1}{m} {\bX}^{\top} \Big( \hat{g}({\bX} \times {\bw}^{(t)}) - \mathbf{y} \Big) \label{eq:unb}
% \end{equation}
% due to the unbiasedness of the truncation protocol. 
From $\mathbb{E}[\mathbf{n}^{(t)}]=0$, we obtain {\color{blue}
\begin{equation}\label{eq:delta}
    \mathbb{E}[\mathbf{p}^{(t)}] - \mathbb{E}[\nabla C(\bw^{(t)})] =\frac{1}{m}\bX^{\top} \mathbb{E}\big[ \hat{g}({\bX}\times {\bw}^{(t)}) - g({\bX}\times {\bw}^{(t)}) \big].  
\end{equation}}
\hspace{-0.11cm}From the Weierstrass approximation theorem~\cite{brinkhuis2011optimization}, for any $\epsilon>0$, there exists a polynomial that approximates the sigmoid arbitrarily well, i.e., $|\hat{g}(x)-g(x)|\leq\epsilon$ for all $x$ in the constrained interval.  
% The domain for the sigmoid function is bounded as $\|\bw\|\leq R$. 
Hence, as there exists a polynomial making the norm of~\eqref{eq:delta} arbitrarily small, {\color{blue}$\mathbb{E}[\mathbf{p}^{(t)}]=\mathbb{E}[\nabla C(\bw^{(t)})]$} and $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{n}^{(t)}  \|^{2}_{2} \big] \leq \sigma^2$. 
% The variance of $\mathbf{p}^{(t)}$ is bounded as $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)}  \|^{2}_{2} \big] \leq \sigma^2$.
% In addition, the variance of $\mathbf{p}^{(t)}$ is bounded as $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)} - \mathbb{E}[\mathbf{v}^{(t)}] \|^{2}_{2} \big] \leq \sigma^2$.

% Let $\mathbf{p}^{(t)} \triangleq \frac{1}{m}{\mathbf{X}}^{\top}(\hat{g}({\mathbf{X}}, {\mathbf{w}}^{(t)}) -\mathbf{y})+\mathbf{v}^{(t)}$ denote the gradient computation of {\acr}. 
% Then, one can show that, (unbiasedness) $\mathbb{E}[\mathbf{p}^{(t)}] = \nabla C (\bw^{(t)})+ \epsilon(r) $ where $\epsilon(r)\rightarrow \mathbf{0}$ as $r\rightarrow\infty$ (see Weierstrass approximation theorem~\cite{brinkhuis2011optimization}) and the expectation is taken with respect to the quantization noises, and (variance bound) $\mathbb{E}\big[\| \mathbf{p}^{(t)} - \mathbb{E}[\mathbf{p}^{(t)}] \|^{2}_{2} \big] = \mathbb{E}\big[\| \mathbf{v}^{(t)} - \mathbb{E}[\mathbf{v}^{(t)}] \|^{2}_{2} \big] \leq \sigma^2$.



% (Convergence)
% Next, we consider the update equation in {\acr} from~\eqref{eq:updateEQN_secret} and prove its convergence to $\bw^{*}$. From the $L$-Lipschitz continuity of $\nabla C({\bw})$ stated in where $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$, we have
Next, we consider the update equation in~\eqref{eq:define_p} and prove its convergence to $\bw^{*}$. From the $L$-Lipschitz continuity of $\nabla C({\bw})$ 
(Theorem 2.1.5 of~\cite{book_Nesterov}), we have
% the gradient of the cross entropy loss function, $\nabla C({\bw})$, we have
\begin{align}
    C(\bw^{(t+1)}) 
    &\!\leq \!C(\bw^{(t)}) \!+\! \langle \nabla C(\bw^{(t)}), \bw^{(t+1)}\!-\!\bw^{(t)}\rangle 
    \!+\! \frac{L}{2}{\| \bw^{(t+1)}\!-\!\bw^{(t)}\! \|}^2  \notag\\
    &\!\leq\! C( \bw^{(t)} )\!-\!\eta \langle \gC ( \bw^{(t)} ), \mathbf{p}^{(t)} \rangle + \frac{L\eta^2}{2}{\| \mathbf{p}^{(t)} \|}^2, \label{eq:Lipschitz_ineq}
\end{align} 
% where $\langle ,\cdot, \rangle$ is the inner product and $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$.
where $\langle ,\cdot, \rangle$ is the inner product. For a cross entropy loss $C(\bw)$, the Lipschitz
constant $L$ is equal to the largest eigenvalue of the Hessian $\nabla^2C(\bw)$ for all $\bw$, and is given by $L=\frac{1}{4}\| {\bX} \|^{2}_{2}$.
{\color{blue}
By taking the expectation on both sides in~\eqref{eq:Lipschitz_ineq}, we have
\begin{align}
    \mathbb{E}\big[ C(\bw^{(t+1)}) \big] 
    &\leq \mathbb{E}\big[C( \bw^{(t)} )\big] - \eta \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big] +\frac{L\eta^2}{2} \big( \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big] + \sigma^2 \big) \label{eq:fisrt_ineq} \\
    &\leq \mathbb{E}\big[C( \bw^{(t)} )\big] - \eta \big(1-\frac{L\eta}{2}\big) \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big]+\frac{L\eta^2\sigma^2}{2} \notag \\
    &\leq \mathbb{E}\big[C( \bw^{(t)} )\big] - \frac{\eta}{2} \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big]\!+\!\frac{\eta\sigma^2}{2} \label{eqn1} \\
    &\leq C(\bw^{*})\!+\!\mathbb{E}\big[\langle \gC ( \bw^{(t)} ), \bw^{(t)} \!-\! \bw^{*}\rangle\big] 
    - \frac{\eta}{2} \mathbb{E}\big[\| \gC ( \bw^{(t)} )\|^2\big]\!+\!\frac{\eta\sigma^2}{2} \label{eqn2}\\
    &\leq C(\bw^{*})+ \mathbb{E}[\langle\mathbf{p}^{(t)},\bw^{(t)} - \bw^{*}\rangle] - \frac{\eta}{2} \mathbb{E}\big[\| \mathbf{p}^{(t)} )\|^2\big]+\eta\sigma^2 \label{eqn3}\\
    &= C(\bw^{*}) +\eta\sigma^2 +\mathbb{E}\Big[ \langle \mathbf{p}^{(t)},\bw^{(t)}-\bw^{*} \rangle-\frac{\eta}{2}\| \mathbf{p}^{(t)} )\|^2\Big] \notag \\
    &=\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \mathbb{E}\| \bw^{(t)} - \bw^{*} \|^2 -\mathbb{E}\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
    % &\leq\! C(\bw^{*}) +\eta\sigma^2 + \frac{1}{2\eta}\big( \| \bw^{(t)} - \bw^{*} \|^2 -\| \bw^{(t+1)} - \bw^{*} )\|^2\big) \label{eqn4}
\end{align}
where~\eqref{eq:fisrt_ineq} holds since $\mathbb{E}[\langle \gC ( \bw^{(t)} ), \mathbf{p}^{(t)}\rangle]=\mathbb{E}[\langle \gC ( \bw^{(t)} ), \gC ( \bw^{(t)} )+\mathbf{n}^{(t)}\rangle]=\mathbb{E}\| \gC ( \bw^{(t)} )\|^2$ and $\mathbb{E}\big[\| \mathbf{p}^{(t)}  - \mathbb{E}[\nabla C(\bw^{(t)})] \|^{2}_{2} \big] \leq \sigma^2$,~\eqref{eqn1} follows from $L\eta\leq1$,~\eqref{eqn2} follows from the convexity of $C$,~\eqref{eqn3} holds since $\mathbb{E}\big[\langle \gC ( \bw^{(t)} ), \bw^{(t)} \!-\! \bw^{*}\rangle\big]=\mathbb{E}\big[\langle \mathbf{p}^{(t)}-\mathbf{n}^{(t)}, \bw^{(t)} \!-\! \bw^{*}\rangle\big]=\mathbb{E}\big[\langle \mathbf{p}^{(t)}, \bw^{(t)} \!-\! \bw^{*}\rangle\big]$ as $\mathbf{n}^{(t)}$ is independent of $\mathbf{w}^{(t)}$ and has zero mean, and \eqref{eqn4} follows from $\mathbf{p}^{(t)}=-\frac{1}{\eta}(\bw^{(t+1)}-\bw^{(t)})$.
}

Summing both sides of the inequality in~\eqref{eqn4} for $t=0,\ldots,J-1$, we find that,
\begin{align*}
    \sum_{t=0}^{J-1}\Big(\mathbb{E}\big[ &C(\bw^{(t+1)})\big]\!-\!C(\bw^{*})\Big) 
    % \notag \\
    % & \leq \frac{1}{2\eta}\big( \| \bw^{(0)} - \bw^{*} \|^2 -\| \bw^{(J)} - \bw^{*} )\|^2\big) + J\eta\sigma^2\\
    \leq \frac{\| \bw^{(0)} - \bw^{*} \|^2}{2\eta}\!+\!J\eta\sigma^2.
\end{align*}
Finally, since $C$ is convex, we observe that, 
\begin{align*}
    \mathbb{E}\Big[ C\big( \frac{1}{J}\sum_{t=0}^{J}\bw^{(t)}\big)\Big]\!-\!C(\bw^{*})
    &\leq \frac{1}{J} \sum_{t=0}^{J-1}\Big(\mathbb{E}\big[ C(\bw^{(t+1)})\big]\!-\!C(\bw^{*})\Big) \notag \\
    &\leq \frac{\| \bw^{(0)} - \bw^{*} \|^2}{2\eta J} + \eta\sigma^2%, 
\end{align*}
which completes the proof of convergence.
